NLO Effects in EFT Fits to $W^+W^-$ Production at the LHC

We study the impact of anomalous gauge boson and fermion couplings on the production of $W^+W^-$ pairs at potential future LHC upgrades and estimate the sensitivity at $\sqrt{S}=14$ TeV with $3~ab^{-1}$ and $\sqrt{S}=27$ TeV with $15~ab^{-1}$. A general technique for including NLO QCD effects in effective field theory (EFT) fits to kinematic distributions is presented, and numerical results are given for $\sqrt{S}=13$ TeV $W^+W^-$ production. Our method allows fits to anomalous couplings at NLO accuracy in any EFT basis and has been implemented in a publicly available version of the POWHEG-BOX. Analytic expressions for the $K$-factors relevant for $13$ TeV total cross sections are given for the HISZ and Warsaw EFT bases and differential $K$-factors can be obtained using the supplemental material. Our study demonstrates the necessity of including anomalous $Z$- fermion couplings in the extraction of limits on anomalous 3-gauge-boson couplings.

==> Untitled-2.tex <==


\begin{table}
\centering
\begin{tabular}{|l|c|c|c|c|c|c|}\hline\hline
$X_{ij}$&2&3&4&5&6&7\\ \hline
$1$ &2.211&-31.35 & -14.67&32.20&36.82 &-10.77\\
$2$ &&-4.963&-2.372&-0.1275&2.931 &0.05577\\
$3$&&&-13.49 &-48.49 &-14.66&9.676\\
$4$&&&&-0.02663&-15.00&-0.02611\\
$5$&&&&&-0.001471&-0.003671\\
$6$&&&&&&$0.0003033$ \\ \hline\hline
\end{tabular}
\caption{Warsaw basis coefficients defined in Eq.(\ref{eq:keff_warsaw}) with ${\vec{C}}=(\delta g_1^Z, \lambda^Z, \delta \kappa^Z, 
\delta g_L^{Zu}, \delta g_R^{Zu},
\delta g_L^{Zd},\delta g_R^{Zd} )$ .}
\label{tab:xfac}
\end{table}
